NICO++: Towards Better Benchmarking for Domain Generalization

Despite the remarkable performance that modern deep neural networks have achieved on independent and identically distributed (I.I.D.) data, they can crash under distribution shifts. Most current evaluation methods for domain generalization (DG) adopt the leave-one-out strategy as a compromise on the limited number of domains. We propose a large-scale benchmark with extensive labeled domains named NICO++ along with more rational evaluation methods for comprehensively evaluating DG algorithms. To evaluate DG datasets, we propose two metrics to quantify covariate shift and concept shift, respectively. Two novel generalization bounds from the perspective of data construction are proposed to prove that limited concept shift and significant covariate shift favor the evaluation capability for generalization. Through extensive experiments, NICO++ shows its superior evaluation capability compared with current DG datasets and its contribution in alleviating unfairness caused by the leak of oracle knowledge in model selection.

==> fancyhdr.tex <==
% fancyhdr.sty version 3.2
% Fancy headers and footers for LaTeX.
% Piet van Oostrum, 
% Dept of Computer and Information Sciences, University of Utrecht,
% Padualaan 14, P.O. Box 80.089, 3508 TB Utrecht, The Netherlands
% Telephone: +31 30 2532180. Email: piet@cs.uu.nl
% ========================================================================
% LICENCE:
% This file may be distributed under the terms of the LaTeX Project Public
% License, as described in lppl.txt in the base LaTeX distribution.
% Either version 1 or, at your option, any later version.
% ========================================================================
% MODIFICATION HISTORY:
% Sep 16, 1994
% version 1.4: Correction for use with \reversemargin
% Sep 29, 1994:
% version 1.5: Added the \iftopfloat, \ifbotfloat and \iffloatpage commands
% Oct 4, 1994:
% version 1.6: Reset single spacing in headers/footers for use with
% setspace.sty or doublespace.sty
% Oct 4, 1994:
% version 1.7: changed \let\@mkboth\markboth to
% \def\@mkboth{\protect\markboth} to make it more robust
% Dec 5, 1994:
% version 1.8: corrections for amsbook/amsart: define \@chapapp and (more
% importantly) use the \chapter/sectionmark definitions from ps@headings if
% they exist (which should be true for all standard classes).
% May 31, 1995:
% version 1.9: The proposed \renewcommand{\headrulewidth}{\iffloatpage...
% construction in the doc did not work properly with the fancyplain style. 
% June 1, 1995:
% version 1.91: The definition of \@mkboth wasn't restored on subsequent
% \pagestyle{fancy}'s.
% June 1, 1995:
% version 1.92: The sequence \pagestyle{fancyplain} \pagestyle{plain}
% \pagestyle{fancy} would erroneously select the plain version.
% June 1, 1995:
% version 1.93: \fancypagestyle command added.
% Dec 11, 1995:
% version 1.94: suggested by Conrad Hughes <chughes@maths.tcd.ie>
% CJCH, Dec 11, 1995: added \footruleskip to allow control over footrule
% position (old hardcoded value of .3\normalbaselineskip is far too high
% when used with very small footer fonts).
% Jan 31, 1996:
% version 1.95: call \@normalsize in the reset code if that is defined,
% otherwise \normalsize.
% this is to solve a problem with ucthesis.cls, as this doesn't
% define \@currsize. Unfortunately for latex209 calling \normalsize doesn't
% work as this is optimized to do very little, so there \@normalsize should
% be called. Hopefully this code works for all versions of LaTeX known to
% mankind.  
% April 25, 1996:
% version 1.96: initialize \headwidth to a magic (negative) value to catch
% most common cases that people change it before calling \pagestyle{fancy}.
% Note it can't be initialized when reading in this file, because
% \textwidth could be changed afterwards. This is quite probable.
% We also switch to \MakeUppercase rather than \uppercase and introduce a
% \nouppercase command for use in headers. and footers.
% May 3, 1996:
% version 1.97: Two changes:
% 1. Undo the change in version 1.8 (using the pagestyle{headings} defaults
% for the chapter and section marks. The current version of amsbook and
% amsart classes don't seem to need them anymore. Moreover the standard
% latex classes don't use \markboth if twoside isn't selected, and this is
% confusing as \leftmark doesn't work as expected.
% 2. include a call to \ps@empty in ps@@fancy. This is to solve a problem
% in the amsbook and amsart classes, that make global changes to \topskip,
% which are reset in \ps@empty. Hopefully this doesn't break other things.
% May 7, 1996:
% version 1.98:
% Added % after the line  \def\nouppercase
% May 7, 1996:
% version 1.99: This is the alpha version of fancyhdr 2.0
% Introduced the new commands \fancyhead, \fancyfoot, and \fancyhf.
% Changed \headrulewidth, \footrulewidth, \footruleskip to
% macros rather than length parameters, In this way they can be
% conditionalized and they don't consume length registers. There is no need
% to have them as length registers unless you want to do calculations with
% them, which is unlikely. Note that this may make some uses of them
% incompatible (i.e. if you have a file that uses \setlength or \xxxx=)
% May 10, 1996:
% version 1.99a:
% Added a few more % signs
% May 10, 1996:
% version 1.99b:
% Changed the syntax of \f@nfor to be resistent to catcode changes of :=
% Removed the [1] from the defs of \lhead etc. because the parameter is
% consumed by the \@[xy]lhead etc. macros.
% June 24, 1997:
% version 1.99c:
% corrected \nouppercase to also include the protected form of \MakeUppercase
% \global added to manipulation of \headwidth.
% \iffootnote command added.
% Some comments added about \@fancyhead and \@fancyfoot.
% Aug 24, 1998
% version 1.99d
% Changed the default \ps@empty to \ps@@empty in order to allow
% \fancypagestyle{empty} redefinition.
% Oct 11, 2000
% version 2.0
% Added LPPL license clause.
%
% A check for \headheight is added. An errormessage is given (once) if the
% header is too large. Empty headers don't generate the error even if
% \headheight is very small or even 0pt. 
% Warning added for the use of 'E' option when twoside option is not used.
% In this case the 'E' fields will never be used.
%
% Mar 10, 2002
% version 2.1beta
% New command: \fancyhfoffset[place]{length}
% defines offsets to be applied to the header/footer to let it stick into
% the margins (if length > 0).
% place is like in fancyhead, except that only E,O,L,R can be used.
% This replaces the old calculation based on \headwidth and the marginpar
% area.
% \headwidth will be dynamically calculated in the headers/footers when
% this is used.
%
% Mar 26, 2002
% version 2.1beta2
% \fancyhfoffset now also takes h,f as possible letters in the argument to
% allow the header and footer widths to be different.
% New commands \fancyheadoffset and \fancyfootoffset added comparable to
% \fancyhead and \fancyfoot.
% Errormessages and warnings have been made more informative.
%
% Dec 9, 2002
% version 2.1
% The defaults for \footrulewidth, \plainheadrulewidth and
% \plainfootrulewidth are changed from \z@skip to 0pt. In this way when
% someone inadvertantly uses \setlength to change any of these, the value
% of \z@skip will not be changed, rather an errormessage will be given.

% March 3, 2004
% Release of version 3.0

% Oct 7, 2004
% version 3.1
% Added '\endlinechar=13' to \fancy@reset to prevent problems with
% includegraphics in header when verbatiminput is active.

% March 22, 2005
% version 3.2
% reset \everypar (the real one) in \fancy@reset because spanish.ldf does
% strange things with \everypar between << and >>.

\def\ifancy@mpty#1{\def\temp@a{#1}\ifx\temp@a\@empty}

\def\fancy@def#1#2{\ifancy@mpty{#2}\fancy@gbl\def#1{\leavevmode}\else
                                   \fancy@gbl\def#1{#2\strut}\fi}

\let\fancy@gbl\global

\def\@fancyerrmsg#1{%
        \ifx\PackageError\undefined
        \errmessage{#1}\else
        \PackageError{Fancyhdr}{#1}{}\fi}
\def\@fancywarning#1{%
        \ifx\PackageWarning\undefined
        \errmessage{#1}\else
        \PackageWarning{Fancyhdr}{#1}{}\fi}

% Usage: \@forc \var{charstring}{command to be executed for each char}
% This is similar to LaTeX's \@tfor, but expands the charstring.

\def\@forc#1#2#3{\expandafter\f@rc\expandafter#1\expandafter{#2}{#3}}
\def\f@rc#1#2#3{\def\temp@ty{#2}\ifx\@empty\temp@ty\else
                                    \f@@rc#1#2\f@@rc{#3}\fi}
\def\f@@rc#1#2#3\f@@rc#4{\def#1{#2}#4\f@rc#1{#3}{#4}}

% Usage: \f@nfor\name:=list\do{body}
% Like LaTeX's \@for but an empty list is treated as a list with an empty
% element

\newcommand{\f@nfor}[3]{\edef\@fortmp{#2}%
    \expandafter\@forloop#2,\@nil,\@nil\@@#1{#3}}

% Usage: \def@ult \cs{defaults}{argument}
% sets \cs to the characters from defaults appearing in argument
% or defaults if it would be empty. All characters are lowercased.

\newcommand\def@ult[3]{%
    \edef\temp@a{\lowercase{\edef\noexpand\temp@a{#3}}}\temp@a
    \def#1{}%
    \@forc\tmpf@ra{#2}%
        {\expandafter\if@in\tmpf@ra\temp@a{\edef#1{#1\tmpf@ra}}{}}%
    \ifx\@empty#1\def#1{#2}\fi}
% 
% \if@in <char><set><truecase><falsecase>
%
\newcommand{\if@in}[4]{%
    \edef\temp@a{#2}\def\temp@b##1#1##2\temp@b{\def\temp@b{##1}}%
    \expandafter\temp@b#2#1\temp@b\ifx\temp@a\temp@b #4\else #3\fi}

\newcommand{\fancyhead}{\@ifnextchar[{\f@ncyhf\fancyhead h}%
                                     {\f@ncyhf\fancyhead h[]}}
\newcommand{\fancyfoot}{\@ifnextchar[{\f@ncyhf\fancyfoot f}%
                                     {\f@ncyhf\fancyfoot f[]}}
\newcommand{\fancyhf}{\@ifnextchar[{\f@ncyhf\fancyhf{}}%
                                   {\f@ncyhf\fancyhf{}[]}}

% New commands for offsets added

\newcommand{\fancyheadoffset}{\@ifnextchar[{\f@ncyhfoffs\fancyheadoffset h}%
                                           {\f@ncyhfoffs\fancyheadoffset h[]}}
\newcommand{\fancyfootoffset}{\@ifnextchar[{\f@ncyhfoffs\fancyfootoffset f}%
                                           {\f@ncyhfoffs\fancyfootoffset f[]}}
\newcommand{\fancyhfoffset}{\@ifnextchar[{\f@ncyhfoffs\fancyhfoffset{}}%
                                         {\f@ncyhfoffs\fancyhfoffset{}[]}}

% The header and footer fields are stored in command sequences with
% names of the form: \f@ncy<x><y><z> with <x> for [eo], <y> from [lcr]
% and <z> from [hf].

\def\f@ncyhf#1#2[#3]#4{%
    \def\temp@c{}%
    \@forc\tmpf@ra{#3}%
        {\expandafter\if@in\tmpf@ra{eolcrhf,EOLCRHF}%
            {}{\edef\temp@c{\temp@c\tmpf@ra}}}%
    \ifx\@empty\temp@c\else
        \@fancyerrmsg{Illegal char `\temp@c' in \string#1 argument:
          [#3]}%
    \fi
    \f@nfor\temp@c{#3}%
        {\def@ult\f@@@eo{eo}\temp@c
         \if@twoside\else
           \if\f@@@eo e\@fancywarning
             {\string#1's `E' option without twoside option is useless}\fi\fi
         \def@ult\f@@@lcr{lcr}\temp@c
         \def@ult\f@@@hf{hf}{#2\temp@c}%
         \@forc\f@@eo\f@@@eo
             {\@forc\f@@lcr\f@@@lcr
                 {\@forc\f@@hf\f@@@hf
                     {\expandafter\fancy@def\csname
                      f@ncy\f@@eo\f@@lcr\f@@hf\endcsname
                      {#4}}}}}}

\def\f@ncyhfoffs#1#2[#3]#4{%
    \def\temp@c{}%
    \@forc\tmpf@ra{#3}%
        {\expandafter\if@in\tmpf@ra{eolrhf,EOLRHF}%
            {}{\edef\temp@c{\temp@c\tmpf@ra}}}%
    \ifx\@empty\temp@c\else
        \@fancyerrmsg{Illegal char `\temp@c' in \string#1 argument:
          [#3]}%
    \fi
    \f@nfor\temp@c{#3}%
        {\def@ult\f@@@eo{eo}\temp@c
         \if@twoside\else
           \if\f@@@eo e\@fancywarning
             {\string#1's `E' option without twoside option is useless}\fi\fi
         \def@ult\f@@@lcr{lr}\temp@c
         \def@ult\f@@@hf{hf}{#2\temp@c}%
         \@forc\f@@eo\f@@@eo
             {\@forc\f@@lcr\f@@@lcr
                 {\@forc\f@@hf\f@@@hf
                     {\expandafter\setlength\csname
                      f@ncyO@\f@@eo\f@@lcr\f@@hf\endcsname
                      {#4}}}}}%
     \fancy@setoffs}

% Fancyheadings version 1 commands. These are more or less deprecated,
% but they continue to work.

\newcommand{\lhead}{\@ifnextchar[{\@xlhead}{\@ylhead}}
\def\@xlhead[#1]#2{\fancy@def\f@ncyelh{#1}\fancy@def\f@ncyolh{#2}}
\def\@ylhead#1{\fancy@def\f@ncyelh{#1}\fancy@def\f@ncyolh{#1}}

\newcommand{\chead}{\@ifnextchar[{\@xchead}{\@ychead}}
\def\@xchead[#1]#2{\fancy@def\f@ncyech{#1}\fancy@def\f@ncyoch{#2}}
\def\@ychead#1{\fancy@def\f@ncyech{#1}\fancy@def\f@ncyoch{#1}}

\newcommand{\rhead}{\@ifnextchar[{\@xrhead}{\@yrhead}}
\def\@xrhead[#1]#2{\fancy@def\f@ncyerh{#1}\fancy@def\f@ncyorh{#2}}
\def\@yrhead#1{\fancy@def\f@ncyerh{#1}\fancy@def\f@ncyorh{#1}}

\newcommand{\lfoot}{\@ifnextchar[{\@xlfoot}{\@ylfoot}}
\def\@xlfoot[#1]#2{\fancy@def\f@ncyelf{#1}\fancy@def\f@ncyolf{#2}}
\def\@ylfoot#1{\fancy@def\f@ncyelf{#1}\fancy@def\f@ncyolf{#1}}

\newcommand{\cfoot}{\@ifnextchar[{\@xcfoot}{\@ycfoot}}
\def\@xcfoot[#1]#2{\fancy@def\f@ncyecf{#1}\fancy@def\f@ncyocf{#2}}
\def\@ycfoot#1{\fancy@def\f@ncyecf{#1}\fancy@def\f@ncyocf{#1}}

\newcommand{\rfoot}{\@ifnextchar[{\@xrfoot}{\@yrfoot}}
\def\@xrfoot[#1]#2{\fancy@def\f@ncyerf{#1}\fancy@def\f@ncyorf{#2}}
\def\@yrfoot#1{\fancy@def\f@ncyerf{#1}\fancy@def\f@ncyorf{#1}}

\newlength{\fancy@headwidth}
\let\headwidth\fancy@headwidth
\newlength{\f@ncyO@elh}
\newlength{\f@ncyO@erh}
\newlength{\f@ncyO@olh}
\newlength{\f@ncyO@orh}
\newlength{\f@ncyO@elf}
\newlength{\f@ncyO@erf}
\newlength{\f@ncyO@olf}
\newlength{\f@ncyO@orf}
\newcommand{\headrulewidth}{0.4pt}
\newcommand{\footrulewidth}{0pt}
\newcommand{\footruleskip}{.3\normalbaselineskip}

% Fancyplain stuff shouldn't be used anymore (rather
% \fancypagestyle{plain} should be used), but it must be present for
% compatibility reasons.

\newcommand{\plainheadrulewidth}{0pt}
\newcommand{\plainfootrulewidth}{0pt}
\newif\if@fancyplain \@fancyplainfalse
\def\fancyplain#1#2{\if@fancyplain#1\else#2\fi}

\headwidth=-123456789sp %magic constant

% Command to reset various things in the headers:
% a.o.  single spacing (taken from setspace.sty)
% and the catcode of ^^M (so that epsf files in the header work if a
% verbatim crosses a page boundary)
% It also defines a \nouppercase command that disables \uppercase and
% \Makeuppercase. It can only be used in the headers and footers.
\let\fnch@everypar\everypar% save real \everypar because of spanish.ldf
\def\fancy@reset{\fnch@everypar{}\restorecr\endlinechar=13
 \def\baselinestretch{1}%
 \def\nouppercase##1{{\let\uppercase\relax\let\MakeUppercase\relax
     \expandafter\let\csname MakeUppercase \endcsname\relax##1}}%
 \ifx\undefined\@newbaseline% NFSS not present; 2.09 or 2e
   \ifx\@normalsize\undefined \normalsize % for ucthesis.cls
   \else \@normalsize \fi
 \else% NFSS (2.09) present
  \@newbaseline%
 \fi}

% Initialization of the head and foot text.

% The default values still contain \fancyplain for compatibility.
\fancyhf{} % clear all
% lefthead empty on ``plain'' pages, \rightmark on even, \leftmark on odd pages
% evenhead empty on ``plain'' pages, \leftmark on even, \rightmark on odd pages
\if@twoside
  \fancyhead[el,or]{\fancyplain{}{\sl\rightmark}}
  \fancyhead[er,ol]{\fancyplain{}{\sl\leftmark}}
\else
  \fancyhead[l]{\fancyplain{}{\sl\rightmark}}
  \fancyhead[r]{\fancyplain{}{\sl\leftmark}}
\fi
\fancyfoot[c]{\rm\thepage} % page number

% Use box 0 as a temp box and dimen 0 as temp dimen. 
% This can be done, because this code will always
% be used inside another box, and therefore the changes are local.

\def\@fancyvbox#1#2{\setbox0\vbox{#2}\ifdim\ht0>#1\@fancywarning
  {\string#1 is too small (\the#1): ^^J Make it at least \the\ht0.^^J
    We now make it that large for the rest of the document.^^J
    This may cause the page layout to be inconsistent, however\@gobble}%
  \dimen0=#1\global\setlength{#1}{\ht0}\ht0=\dimen0\fi
  \box0}

% Put together a header or footer given the left, center and
% right text, fillers at left and right and a rule.
% The \lap commands put the text into an hbox of zero size,
% so overlapping text does not generate an errormessage.
% These macros have 5 parameters:
% 1. LEFTSIDE BEARING % This determines at which side the header will stick
%    out. When \fancyhfoffset is used this calculates \headwidth, otherwise
%    it is \hss or \relax (after expansion).
% 2. \f@ncyolh, \f@ncyelh, \f@ncyolf or \f@ncyelf. This is the left component.
% 3. \f@ncyoch, \f@ncyech, \f@ncyocf or \f@ncyecf. This is the middle comp.
% 4. \f@ncyorh, \f@ncyerh, \f@ncyorf or \f@ncyerf. This is the right component.
% 5. RIGHTSIDE BEARING. This is always \relax or \hss (after expansion).

\def\@fancyhead#1#2#3#4#5{#1\hbox to\headwidth{\fancy@reset
  \@fancyvbox\headheight{\hbox
    {\rlap{\parbox[b]{\headwidth}{\raggedright#2}}\hfill
      \parbox[b]{\headwidth}{\centering#3}\hfill
      \llap{\parbox[b]{\headwidth}{\raggedleft#4}}}\headrule}}#5}

\def\@fancyfoot#1#2#3#4#5{#1\hbox to\headwidth{\fancy@reset
    \@fancyvbox\footskip{\footrule
      \hbox{\rlap{\parbox[t]{\headwidth}{\raggedright#2}}\hfill
        \parbox[t]{\headwidth}{\centering#3}\hfill
        \llap{\parbox[t]{\headwidth}{\raggedleft#4}}}}}#5}

\def\headrule{{\if@fancyplain\let\headrulewidth\plainheadrulewidth\fi
    \hrule\@height\headrulewidth\@width\headwidth \vskip-\headrulewidth}}

\def\footrule{{\if@fancyplain\let\footrulewidth\plainfootrulewidth\fi
    \vskip-\footruleskip\vskip-\footrulewidth
    \hrule\@width\headwidth\@height\footrulewidth\vskip\footruleskip}}

\def\ps@fancy{%
\@ifundefined{@chapapp}{\let\@chapapp\chaptername}{}%for amsbook
%
% Define \MakeUppercase for old LaTeXen.
% Note: we used \def rather than \let, so that \let\uppercase\relax (from
% the version 1 documentation) will still work.
%
\@ifundefined{MakeUppercase}{\def\MakeUppercase{\uppercase}}{}%
\@ifundefined{chapter}{\def\sectionmark##1{\markboth
{\MakeUppercase{\ifnum \c@secnumdepth>\z@
 \thesection\hskip 1em\relax \fi ##1}}{}}%
\def\subsectionmark##1{\markright {\ifnum \c@secnumdepth >\@ne
 \thesubsection\hskip 1em\relax \fi ##1}}}%
{\def\chaptermark##1{\markboth {\MakeUppercase{\ifnum \c@secnumdepth>\m@ne
 \@chapapp\ \thechapter. \ \fi ##1}}{}}%
\def\sectionmark##1{\markright{\MakeUppercase{\ifnum \c@secnumdepth >\z@
 \thesection. \ \fi ##1}}}}%
%\csname ps@headings\endcsname % use \ps@headings defaults if they exist
\ps@@fancy
\gdef\ps@fancy{\@fancyplainfalse\ps@@fancy}%
% Initialize \headwidth if the user didn't
%
\ifdim\headwidth<0sp
%
% This catches the case that \headwidth hasn't been initialized and the
% case that the user added something to \headwidth in the expectation that
% it was initialized to \textwidth. We compensate this now. This loses if
% the user intended to multiply it by a factor. But that case is more
% likely done by saying something like \headwidth=1.2\textwidth. 
% The doc says you have to change \headwidth after the first call to
% \pagestyle{fancy}. This code is just to catch the most common cases were
% that requirement is violated.
%
    \global\advance\headwidth123456789sp\global\advance\headwidth\textwidth
\fi}
\def\ps@fancyplain{\ps@fancy \let\ps@plain\ps@plain@fancy}
\def\ps@plain@fancy{\@fancyplaintrue\ps@@fancy}
\let\ps@@empty\ps@empty
\def\ps@@fancy{%
\ps@@empty % This is for amsbook/amsart, which do strange things with \topskip
\def\@mkboth{\protect\markboth}%
\def\@oddhead{\@fancyhead\fancy@Oolh\f@ncyolh\f@ncyoch\f@ncyorh\fancy@Oorh}%
\def\@oddfoot{\@fancyfoot\fancy@Oolf\f@ncyolf\f@ncyocf\f@ncyorf\fancy@Oorf}%
\def\@evenhead{\@fancyhead\fancy@Oelh\f@ncyelh\f@ncyech\f@ncyerh\fancy@Oerh}%
\def\@evenfoot{\@fancyfoot\fancy@Oelf\f@ncyelf\f@ncyecf\f@ncyerf\fancy@Oerf}%
}
% Default definitions for compatibility mode:
% These cause the header/footer to take the defined \headwidth as width
% And to shift in the direction of the marginpar area

\def\fancy@Oolh{\if@reversemargin\hss\else\relax\fi}
\def\fancy@Oorh{\if@reversemargin\relax\else\hss\fi}
\let\fancy@Oelh\fancy@Oorh
\let\fancy@Oerh\fancy@Oolh

\let\fancy@Oolf\fancy@Oolh
\let\fancy@Oorf\fancy@Oorh
\let\fancy@Oelf\fancy@Oelh
\let\fancy@Oerf\fancy@Oerh

% New definitions for the use of \fancyhfoffset
% These calculate the \headwidth from \textwidth and the specified offsets.

\def\fancy@offsolh{\headwidth=\textwidth\advance\headwidth\f@ncyO@olh
                   \advance\headwidth\f@ncyO@orh\hskip-\f@ncyO@olh}
\def\fancy@offselh{\headwidth=\textwidth\advance\headwidth\f@ncyO@elh
                   \advance\headwidth\f@ncyO@erh\hskip-\f@ncyO@elh}

\def\fancy@offsolf{\headwidth=\textwidth\advance\headwidth\f@ncyO@olf
                   \advance\headwidth\f@ncyO@orf\hskip-\f@ncyO@olf}
\def\fancy@offself{\headwidth=\textwidth\advance\headwidth\f@ncyO@elf
                   \advance\headwidth\f@ncyO@erf\hskip-\f@ncyO@elf}

\def\fancy@setoffs{%
% Just in case \let\headwidth\textwidth was used
  \fancy@gbl\let\headwidth\fancy@headwidth
  \fancy@gbl\let\fancy@Oolh\fancy@offsolh
  \fancy@gbl\let\fancy@Oelh\fancy@offselh
  \fancy@gbl\let\fancy@Oorh\hss
  \fancy@gbl\let\fancy@Oerh\hss
  \fancy@gbl\let\fancy@Oolf\fancy@offsolf
  \fancy@gbl\let\fancy@Oelf\fancy@offself
  \fancy@gbl\let\fancy@Oorf\hss
  \fancy@gbl\let\fancy@Oerf\hss}

\newif\iffootnote
\let\latex@makecol\@makecol
\def\@makecol{\ifvoid\footins\footnotetrue\else\footnotefalse\fi
\let\topfloat\@toplist\let\botfloat\@botlist\latex@makecol}
\def\iftopfloat#1#2{\ifx\topfloat\empty #2\else #1\fi}
\def\ifbotfloat#1#2{\ifx\botfloat\empty #2\else #1\fi}
\def\iffloatpage#1#2{\if@fcolmade #1\else #2\fi}

\newcommand{\fancypagestyle}[2]{%
  \@namedef{ps@#1}{\let\fancy@gbl\relax#2\relax\ps@fancy}}

